Reverse Engineering of Irreducible Polynomials in GF(2^m) Arithmetic

Current techniques for formally verifying circuits implemented in Galois field (GF) arithmetic are limited to those with a known irreducible polynomial P(x). This paper presents a computer algebra based technique that extracts the irreducible polynomial P(x) used in the implementation of a multiplier in GF(2^m). The method is based on first extracting a unique polynomial in Galois field of each output bit independently. P(x) is then obtained by analyzing the algebraic expression in GF(2^m) of each output bit. We demonstrate that this method is able to reverse engineer the irreducible polynomial of an n-bit GF multiplier in n threads. Experiments were performed on Mastrovito and Montgomery multipliers with different P (x), including NIST-recommended polynomials and optimal polynomials for different microprocessor architectures.

==> 2-bit-rewritting.tex <==
\begin{figure}[]
\centering
%\scriptsize
\small
\begin{tabular}{|l|c|}
\hline
$Sig_{out}$: $F_0$=$z_0$+x$z_1$                                                &  Eliminating terms           \\ \hline
G7: $F_1$=$z_0$+x($n_5$+$n_6$)                                             & \textit{-}  \\ \hline
G6: $F_2$=$n_1$+$n_2$+x($n_5$+$n_6$)                                           & \textit{-}  \\ \hline
G5: $F_3$=$n_1$+$n_2$+x($n_3$+$n_4$+$n_5$)                                     & \textit{-}  \\ \hline
G8: $F_4$=$n_1$+$n_2$+x($n_3$+$n_4$+$n_2$+1)                                   & \textit{-}  \\ \hline
G4: $F_5$=$n_1$+$n_2$+x($n_2$+$n_3$+$a_0$$b_1$)+2x                          & \textit{2x} \\ \hline
G3: $F_6$=$n_1$+$n_2$+x($n_2$+$a_1$$b_0$+$a_0$$b_1$+1)                      & \textit{-}  \\ \hline
G2: $F_7$=$n_1$+$a_1$$b_1$+1+x($a_1$$b_1$+$a_1$$b_0$+$a_0$$b_1$)+2x      & \textit{2x} \\ \hline
G1: $F_8$=$a_0$$b_0$+$a_1$$b_1$+2+x($a_1$$b_1$+$a_1$$b_0$+$a_0$$b_1$) & \textit{2}  \\ \hline
$Sig_{in}$: $a_0$$b_0$+$a_1$$b_1$+x($a_1$$b_1$+$a_1$$b_0$+$a_0$$b_1$) & \textit{-}  \\ \hline
\end{tabular}
\caption{Function extraction of a 2-bit $GF$ multiplier shown in Figure 2 using backward rewiring from PO to PI.}
\label{fig:rewriting}
\end{figure}


==> 4-bit-p_x_comparison.tex <==
\begin{figure}[!htb]
\centering
%\caption{My caption}
\begin{tabular}{lllllll}
     &      &      & $a_3$   & $a_2$   & $a_1$   & $a_0$   \\
     &      &      & $b_3$   & $b_2$   & $b_1$   & $b_0$   \\ \hline
     &      &      & $a_{3}b_{0}$ & $a_{2}b_{0}$ & $a_{1}b_{0}$ & $a_{0}b_{0}$ \\
     &      & $a_{3}b_{1}$ & $a_{2}b_{1}$ & $a_{1}b_{1}$ & $a_{0}b_{1}$ &  \\
     & $a_{3}b_{2}$ & $a_{2}b_{2}$ & $a_{1}b_{2}$ & $a_{0}b_{2}$  &      &      \\
$a_{3}b_{3}$ & $a_{2}b_{3}$ & $a_{1}b_{3}$ & $a_{0}b_{3}$  &      &      &      \\ \hline
$s_6$   & $s_5$   & $s_4$   & $s_3$   & $s_2$   & $s_1$   & $s_0$  \\
\end{tabular}
\vspace{2mm}
        \begin{minipage}{.5\linewidth}
      %\caption{$P(x)$=$x^{4}+x^{3}+1$}
      \centering
\begin{tabular}{cccc}
\multicolumn{4}{l}{$P(x)$=$x^{4}+x^{3}+1$}                                                                            \\
\multicolumn{1}{c|}{$s_3$} & \multicolumn{1}{c|}{$s_2$} & \multicolumn{1}{c|}{$s_1$} & $s_0$                     \\
\multicolumn{1}{c|}{$s_4$} & \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{0} & $s_4$                     \\
\multicolumn{1}{c|}{$s_5$} & \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{$s_5$}  & $s_5$                     \\
\multicolumn{1}{c|}{$s_6$} & \multicolumn{1}{c|}{$s_6$} & \multicolumn{1}{c|}{$s_6$}  & $s_6$                      \\ \hline
\multicolumn{1}{l|}{$z_3$} & \multicolumn{1}{l|}{$z_2$} & \multicolumn{1}{l|}{$z_1$} & \multicolumn{1}{l}{$z_0$}
\end{tabular}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
        %\caption{$P(x)$=$x^{4}+x+1$}
\begin{tabular}{cccc}
\multicolumn{4}{l}{$P(x)$=$x^{4}+x+1$}                                                                            \\
\multicolumn{1}{c|}{$s_3$} & \multicolumn{1}{c|}{$s_2$} & \multicolumn{1}{c|}{$s_1$} & $s_0$                     \\
\multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{$s_4$} & $s_4$                     \\
\multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{$s_5$}  & \multicolumn{1}{c|}{$s_5$}  & 0                     \\
\multicolumn{1}{c|}{$s_6$} & \multicolumn{1}{c|}{$s_6$} & \multicolumn{1}{c|}{0}  & 0                      \\ \hline
\multicolumn{1}{l|}{$z_3$} & \multicolumn{1}{l|}{$z_2$} & \multicolumn{1}{l|}{$z_1$} & \multicolumn{1}{l}{$z_0$}
\end{tabular}    \end{minipage} 
\caption{Analysis of the computation complexity of Galois field multipliers with different irreducible polynomials using two 4-bit GF multiplications, which are implemented using $x^{4}+x^{3}+1$ and $x^{4}+x+1$.}
\label{fig:study}
\end{figure}



==> conclusion.tex <==
\section{Conclusion}




==> implementation.tex <==
%\section{Parallel Verification} \label{sec:parallel}
\section{Implementation} \label{sec:implementation}

\begin{figure}[!htb] 
\begin{center}
\includegraphics[scale=0.5]{../figs/flow.eps}
\caption{Overview of parallel verification of GF multipliers.}
\label{fig:flow}
\end{center}
\end{figure}

\input{../results/mas_mult_results}
\input{../results/mont_mult_results}


This section describes the implementation of our parallel verification method for Galois field multipliers. The overview of the proposed technique is shown in Figure \ref{fig:flow}. Our approach takes the gate-level netlist as input, and outputs the extracted function of the design. It includes four steps: 
\begin{enumerate}
\item Converting the gate-level netlist into algebraic equations. During this step, the gate-level netlist is translated into algebraic equations based on Eq.(1). The equations are levelized in topological order, to be rewritten by backward rewriting in the next step.
%
\item Splitting the output signature of $GF(2^{m})$ multipliers into $m$ polynomials with $Sig_{out\_i}$=$z_{i}$. These new \textit{signatures} are represented by $m$ equation files.
%
\item Splitting the function of $m$ output bits into $m$ separate functions, each to be processed by a separate thread using Algorithm 1. In contrast to work of \cite{ciesielski2015verification}, the internal expression of each output bit does not provide any polynomial reduction (\textit{monomial cancellations} for other bits.
%
\item Computing the final function of the multiplier. Once the algebraic expression of each output bit in $GF(2)$ is computed, our method computes the final function by substituting the output variables in the $Sig_{out}$ with the corresponding expressions computed in step 3.


\end{enumerate}
\input{../figs/parallel_example.tex}

{\bf Example 2} (Figure \ref{fig:parallel}): We illustrate our parallel extraction method using the 2-bit multiplier in $GF(2^2)$ in Figure \ref{fig:netlist-2bit}. The output signature $Sig_{out}$ = $z_0$+$z_{1}x$ is split into two signatures, $Sig_{out0}=z_0$ and $Sig_{out1}=z_1$. Then, the rewriting process is applied to $Sig_{out0}$ and $Sig_{out1}$ in parallel. When $Sig_{out0}$ and $Sig_{out1}$ have been successfully extracted, the signatures is merged resulting in the polynomial $Sig_{in}$. In Figure 3, we can see that elimination happens three times ($F_5$, $F_7$, and $F_8$). According to Theorem 3, we know that the elimination happens within each element in GF($2^n$). In Figure \ref{fig:parallel}, one elimination in $Sig_{out0}$ and two eliminations in $Sig_{out1}$ have been done independently, which matches the result shown earlier (Figure 3). 












